These Deals Won't Last! Longevity, Uniformity and Bias in Product Badge Assignment in E-Commerce Platforms

Product badges are ubiquitous in e-commerce platforms, acting as effective psychological triggers to nudge customers to buy specific products, boosting revenues. However, to the best of our knowledge, there has been no attempt to systematically study these badges and their several idiosyncrasies - we intend to close this gap in our current work. Specifically, we try to answer questions such as: How long does a product retain a badge on a given platform? If a product is sold on different platforms, then does it receive similar badges? How do the products that receive badges differ from those which do not, in terms of price, customer rating, etc. We collect longitudinal data from several e-commerce platforms over 45 days, and find that although most of the badges are short-lived, there are several permanent badge assignments and that too for badges meant to denote urgency or scarcity. Furthermore, it is unclear how the badge assignments are done, and we find evidence that highly-rated products are missing out on badges compared to lower quality ones. Our work calls for greater transparency in the badge assignment process to inform customers, as well as to reduce dissatisfaction among the sellers dependent on the platforms for their revenues.

==> archit_table.tex <==
\begin{table}[tbh]
\centering
%\setlength{\tabcolsep}{2pt}
\resizebox{.85\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|}
\hline
{\bf Website} & {\bf Product} & {\bf Badge} & {\bf Consistency}\\
\hline
Bewakoof & Women's Sleeveless Button Down Mandarin Collar Side Slit Kurta & Few Left & 1.0 \\
Bewakoof & Jet Black Plain Sleeveless Puffer Jacket with Detachable Hood & Few Left & 1.0 \\
%Bewakoof & Style Quotient Women Olive Green Boxy Solid Casual Shirt & Few Left & 1.0 \\
Bewakoof & Women's Rib Raglan Dress & Buy X Get Y & 1.0 \\
%Bewakoof & Gibral Tar Sea Mandarin Collar Half Sleeve Shirt & Buy X Get Y & 1.0 \\
FirstCry & Baby Peony Dress Set & X Left & 1.0 \\
FirstCry & TINY BABY Sleeveless Checked Dress & X Left & 1.0 \\
%Hopscotch & Kitty Pink Animal Hooded Towel & X Left & 1.0 \\
Hopscotch & Pink Flower Lace Onesies with Headband & X Left & 1.0 \\
Hopscotch & Navy Blue LED Shoes & X Left & 1.0 \\
My Baby Babbles & 3 Sprouts Stroller Organiser & Sale & 1.0 \\
My Baby Babbles & My Milestones Baby Hooded Towel - Modern Stripped & Sale & 1.0 \\
Snapdeal & Mars 2in1 Makeup Fixer Spray & Face Primer Gel & X Left! & 1.0 \\
Snapdeal & Mee Mee Pram Cum Stroller With Rocking Function & X Left! & 1.0 \\
e.l.f. Cosmetics & No Budge Precision Eyeliner & New & 1.0 \\
e.l.f. Cosmetics & Jelly Poppin' Skincare Set & New & 1.0 \\
Max Fashion & MAX Printed Straight Kurta & New & 1.0 \\
Max Fashion & MAX Solid Slim Fit Casual Shirt & New & 1.0 \\
%Max Fashion & MAX Solid Skinny Fit Chinost & New & 1.0 \\
%Max Fashion & MAX Stonewashed Denim Jacket & New & 1.0 \\
%Max Fashion & MAX Solid Skinny Fit Jeans & New & 1.0 \\
\hline
\end{tabular}}
\caption{\bf .}
\label{tab:archit_table}
\end{table}

==> old_introduction.tex <==
\section{Introduction}
\label{sec:intro}
\noindent If one logs into an e-commerce website and searches for a product, then (s)he will inevitably find that the recommendation list contains some products which are highlighted with badges, such as, `Best Seller', `Deal of the Day', `New Arrival', `Discount'.
All these badges evoke specific psychological reactions in a customer; for example, a `Best Seller' badge means that many other customers have already bought this popular product and hence any doubt that the current customer may have regarding its utility is put to rest, whereas `Deal of the Day' creates a sense of urgency that the customer may miss out on a wonderful opportunity if that item is not bought today itself.

\begin{table*}[t!]
\centering
\resizebox{.95\linewidth}{!}{
\begin{tabular}{|l|p{3.5cm}|p{11cm}|}
\hline
{\bf Domain}  & {\bf Niche Websites}               & {\bf Search Queries}\\
\hline
Baby Products & FirstCry, Hopscotch, My Baby Babbles  
& Baby diaper, Baby toys, Baby boy clothes, Stroller, Baby towel, Baby shampoo, Baby girl dresses, Onesies, Baby footwear, Baby food \\ \hline
Cosmetics & e.l.f. Cosmetics, Nykaa 
& Eyeliner, Lipstick, Blush, Cleanser, Moisturizer, Face primer, Makeup removers, Face brush, Lip balm, Mascara \\ \hline
Fashion & Bewakoof, LimeRoad, Max Fashion 
& Women dresses, Women kurtis, Women jackets, Women jeans, Women shirts, Men casual shirts, Men trousers, Men polo t-shirts, Men socks, Men track pants \\ \hline
Home Decor & Pepperfry, Urban Ladder 
& Bed, Dining set, Mattress, Bedsheet, Table lamp, Sofa set, Study table, Wall mirror, Chair, Artificial plants \\
\hline \hline
{\bf Domain}  & {\bf Generic Websites}               & {\bf Search Queries} \\ \hline
All four & Amazon, Snapdeal & All queries mentioned above \\
\hline
\end{tabular}}
\caption{\bf Data collection: e-commerce websites from different domains and the queries used to collect product listing.}
\label{tab:niche}
\end{table*}

There seems to be little study done on the badges that are given on websites.
In~\cite{superhostAirbnb}, the author looks into how the `SuperHost' badge in Airbnb helps improve sales at a higher charge.
Related to e-commerce, the work reported in~\cite{hallOfFameAmazon} covers how Amazon persuades its customers to write more reviews by giving the `Hall of Fame' badge.
The authors of~\cite{hallOfFameAmazon} have further looked into various persuasive strategies that are employed in e-commerce in~\cite{persuasive20,persuasive21}; however, they seem to have never studied product badges which are a common sight across all e-commerce platforms, and can be effective towards persuading customers to choose one product over others.
This book~\cite{influenceBook} is a pioneering work in the field of intersection between human psychology and marketing, and many of the marketing strategies including product badges seem to be inspired from this work.
The blog~\cite{badgeBlog} gives a comprehensive view of the different badges that are displayed on e-commerce platforms, and our categorization scheme for badges borrows from this line of work.
However, there seems to be no work regarding the longevity of product badges, how uniformly does a product receive a badge across platforms, or how do the products with badges vary from those without these.
It may be worth noting that we use the terms `website' and `platform', and `product' and `item' synonymously throughout the paper.

In this work, we look into different niche markets, and investigate websites that cater to these niche markets only, along with generic websites that include a wide variety of products including the niche market.
Specifically, we try to answer the following research questions:
\begin{itemize}
\item[] \textbf{RQ1:} How can we effectively categorize product badges?
\item[] \textbf{RQ2:} Do product badges follow similar or different trends based on whether the platform is generic or niche?
\item[] \textbf{RQ3:} Do product badges follow similar or different trends based on the market it serves?
\item[] \textbf{RQ4:} How long does a product retain a badge on a given platform?
\item[] \textbf{RQ5:} How does the longevity of the badge depend on the platform type, market type and badge type?
\item[] \textbf{RQ6:} If a product is sold on different platforms, then does it receive similar badges?
\item[] \textbf{RQ7:} How do the products that receive badges differ from those which do not, in terms of price, customer rating, etc.?
\end{itemize}

\iffalse
The paper is organized as follows.
Section~\ref{sec:data} explains our data collection process.
Section~\ref{sec:category} covers how we categorize the different badges.
Section~\ref{sec:results} provides our experimental results.
Section~\ref{sec:concl} concludes the paper.
\fi
